Tracing the Arrow of Time: Diagnosing Temporal Information Flow in Video-LLMs

The Arrow-of-Time (AoT) task, determining whether a video plays forward or backward by recognizing temporal irreversibility, is one humans solve with near-perfect accuracy, yet frontier Video Large Language Models (Video-LLMs) perform only modestly above chance. This gap raises a key question: do visual backbones fail to encode temporal information, or does information bottleneck lie elsewhere in the Video-LLM architecture? We address this question by isolating the vision encoder from the Video-LLM and tracing temporal information across the encoder, projector, and LLM. We find that video-centric encoders with explicit temporal modeling encode strong temporal signals, whereas frame-centric encoders do not. However, when video-centric representations are passed through a standard Video-LLM architecture, performance often collapses, revealing a bottleneck of temporal information flow. We identify projector design as a key factor: Q-Former disrupts temporal information, while a time-preserved MLP projection substantially improves the LLM's access to such information. Our layer-wise analysis further shows temporal representation dynamics across encoder layers. Guided by these findings, we build a Video-LLM with temporal-aware video-centric encoder, time-preserved projector, and AoT supervision, surpassing human performance on AoT$_{PPB}$ with 98.1\% accuracy, and improving broader temporal reasoning tasks by up to 6.0 points on VITATECS-Direction and 1.3 points on TVBench. Our results show that temporal reasoning in Video-LLMs requires both effective temporal encoding and reliable transfer of this information to the LLM.

==> tables/lora_it.tex <==
\definecolor{stageone}{RGB}{54,95,145}
\definecolor{stageonebg}{RGB}{235,242,250}
\definecolor{stagetwo}{RGB}{196,114,36}
\definecolor{stagetwobg}{RGB}{252,241,228}
\definecolor{gaincolor}{RGB}{34,139,34}
\definecolor{degradecolor}{RGB}{190,60,60}
\definecolor{neutralcolor}{RGB}{120,120,120}

\begin{table}[t]
\centering
\caption{\textbf{Instruction-Tuning Data Ablation on AoT$_{PPB}$.} We compare general instruction tuning data (I), AoT VQA data (A), and their combination (I+A) across different visual encoders and LLM backbones. Colored deltas indicate the accuracy change relative to the corresponding instruction-only baseline.}
\label{tab:it_ablation}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcl}
\toprule
\textbf{Model} & \textbf{Data} & \textbf{Acc. ($\Delta$)} \\
\midrule

Mistral-7B \\

\rowcolor{stageonebg}
\qquad+ \textcolor{stageone}{InternVideo2$_{\textit{stage1}}$} 
& I 
& 48.6 {\scriptsize \textcolor{neutralcolor}{($-$)}} \\

\rowcolor{stageonebg}
\qquad+ \textcolor{stageone}{InternVideo2$_{\textit{stage1}}$} 
& A 
& 95.1 {\scriptsize \textcolor{gaincolor}{(+46.5)}}  \\

\rowcolor{stageonebg}
\qquad+ \textcolor{stageone}{InternVideo2$_{\textit{stage1}}$} 
& I+A 
& 94.8 {\scriptsize \textcolor{gaincolor}{(+46.2)}} \\

\rowcolor{stagetwobg}
\qquad+ \textcolor{stagetwo}{InternVideo2$_{\textit{stage2}}$} 
& I 
& 50.0 {\scriptsize \textcolor{neutralcolor}{($-$)}}\\

\rowcolor{stagetwobg}
\qquad+ \textcolor{stagetwo}{InternVideo2$_{\textit{stage2}}$} 
& A 
& 73.1 {\scriptsize \textcolor{gaincolor}{(+23.1)}}  \\

\rowcolor{stagetwobg}
\qquad+ \textcolor{stagetwo}{InternVideo2$_{\textit{stage2}}$} 
& I+A 
& 79.3 {\scriptsize \textcolor{gaincolor}{(+29.3)}}  \\

\midrule

Qwen2.5-7B \\

\rowcolor{stageonebg}
\qquad+ \textcolor{stageone}{InternVideo2$_{\textit{stage1}}$} 
& I 
& 50.7 {\scriptsize \textcolor{neutralcolor}{($-$)}}\\

\rowcolor{stageonebg}
\qquad+ \textcolor{stageone}{InternVideo2$_{\textit{stage1}}$} 
& A 
& 96.2 {\scriptsize \textcolor{gaincolor}{(+45.5)}} \\

\rowcolor{stageonebg}
\qquad+ \textcolor{stageone}{InternVideo2$_{\textit{stage1}}$} 
& I+A 
& \textbf{98.1} {\scriptsize \textcolor{gaincolor}{(+47.4)}} \\

\rowcolor{stagetwobg}
\qquad+ \textcolor{stagetwo}{InternVideo2$_{\textit{stage2}}$} 
& I 
& 41.0 {\scriptsize \textcolor{neutralcolor}{($-$)}}\\

\rowcolor{stagetwobg}
\qquad+ \textcolor{stagetwo}{InternVideo2$_{\textit{stage2}}$} 
& A 
& 75.2 {\scriptsize \textcolor{gaincolor}{(+34.2)}} \\

\rowcolor{stagetwobg}
\qquad+ \textcolor{stagetwo}{InternVideo2$_{\textit{stage2}}$} 
& I+A 
& 82.6 {\scriptsize \textcolor{gaincolor}{(+41.6)}} \\

\bottomrule
\end{tabular}
\end{table}
